Designing FPT algorithms for cut problems using randomized contractions

We introduce a new technique for designing fixed-parameter algorithms for cut problems, namely randomized contractions. We apply our framework to obtain the first FPT algorithm for the Unique Label Cover problem and new FPT algorithms with exponential speed up for the Steiner Cut and Node Multiway Cut-Uncut problems. More precisely, we show the following: - We prove that the parameterized version of the Unique Label Cover problem, which is the base of the Unique Games Conjecture, can be solved in 2^{O(k^2\log |\Sigma|)}n^4\log n deterministic time (even in the stronger, vertex-deletion variant) where k is the number of unsatisfied edges and |\Sigma| is the size of the alphabet. As a consequence, we show that one can in polynomial time solve instances of Unique Games where the number of edges allowed not to be satisfied is upper bounded by O(\sqrt{\log n}) to optimality, which improves over the trivial O(1) upper bound. - We prove that the Steiner Cut problem can be solved in 2^{O(k^2\log k)}n^4\log n deterministic time and \tilde{O}(2^{O(k^2\log k)}n^2) randomized time where k is the size of the cutset. This result improves the double exponential running time of the recent work of Kawarabayashi and Thorup (FOCS'11). - We show how to combine considering `cut' and `uncut' constraints at the same time. More precisely, we define a robust problem Node Multiway Cut-Uncut that can serve as an abstraction of introducing uncut constraints, and show that it admits an algorithm running in 2^{O(k^2\log k)}n^4\log n deterministic time where k is the size of the cutset. To the best of our knowledge, the only known way of tackling uncut constraints was via the approach of Marx, O'Sullivan and Razgon (STACS'10), which yields algorithms with double exponential running time. An interesting aspect of our technique is that, unlike important separators, it can handle real weights.

==> conclusions.tex <==
\section{Conclusions}\label{sec:conclusions}

In this paper we presented a new technique of designing parameterized algorithms for cut problems. The natural next step is to try to find further applications of this framework. 
In particular, we would like to ask whether it is possible to provide an algorithm for \multicut parameterized by the size of the cutset only using our framework? To the best of our knowledge, both the approaches of Marx and Razgon~\cite{marx:multicut} and of Bousquet et al.~\cite{thomasse:multicut} do not extend easily to the variants with real weights. Maybe it is possible to solve weighted variant of \multicut using our techniques.

On the other hand, the algorithms obtained using our framework run in time complexity $2^{O(k^2\log k)}\cdot \textrm{poly}(n)$.
Very recently, Wahlstr\"{o}m obtained a single-exponential algorithm for the edge-deletion variant of \ulc, using significantly different methods \cite{magnus:lp}.
Can we obtain better dependency on $k$ in the running time for the other
problems considered in our work? In particular, can we find ``good separations'' more efficiently?


%Is the dependence on $k$ optimal (for example, under Exponential Time Hypothesis)? Or is it possible to design algorithms with running time $2^{O(k\log k)}\cdot \textrm{poly}(n)$ or even $2^{O(k)}\cdot \textrm{poly}(n)$ for at least some of the considered problems?

%In this paper we presented a new technique of designing parameterized algorithms for cut problems. The natural next step is to try to find further applications of this framework. In particular, the following two problems are in our opinion of high interest.
%
%\begin{itemize}
%\item Is it possible to provide an algorithm for \multicut parameterized by the size of the cutset only using our framework? To the best of our knowledge, both the approaches of Marx and Razgon~\cite{marx:multicut} and of Bousquet et al.~\cite{thomasse:multicut} do not extend easily to the variants with real weights. Maybe it is possible to solve weighted variant of \multicut using our techniques.
%\item In the \bisection problem one is given an undirected graph with even number of vertices and an integer $k$. The question is whether there exists a cutset consisting of at most $k$ edges that separates the graph into parts of equal size. To the best of our knowledge, the parameterized complexity of \bisection parameterized by $k$ is open. Is it possible to use our techniques in this problem?
%\item The algorithms obtained from our framework work in time complexity $2^{O(k^2\log k)}\cdot \textrm{poly}(n)$. Is the dependece on $k$ optimal (for example, under Exponential Time Hypothesis)? Or is it possible to design algorithms with running time $2^{O(k\log k)}\cdot \textrm{poly}(n)$ or even $2^{O(k)}\cdot \textrm{poly}(n)$ for at least some of the considered problems?
%\end{itemize}



==> full-ulc-smietnik.tex <==
Instead of using the notion of steps, where the steps were applied sequentially to the instance,
we present in this section the algorithm as 
a set of reduction and branching rules; at each moment, the lowest-numbered applicable
rule is applied.
\begin{itemize}
\item In a {\em{reduction rule}}, we perform some operations to add new elements to
the elements of the tuple $(X_0,S,S^\Psi,\Psi^S)$.
\item In a {\em{branching rule}}, we branch into at most $O(s+\cutsize)$ subcases;
in each subcase we add at least one new element to the set $X_0$.
\end{itemize}
Note that the search tree generated by the algorithm has at most $2^{O(\cutsize \log (s + \cutsize))}$ leaves, if we terminate the computation whenever $|X_0| \geq \cutsize$
(see Rule \ref{rule:ulc-negative-k}).

Given a tuple $(X_0,S,S^\Psi,\Psi^S)$, we denote $D = V(G) \setminus (X_0 \cup S)$;
the algorithm has not yet decided whether the vertices of $D$ should be included in
a deletion set.
We start with some obvious reduction rules.
\begin{redrule}\label{rule:ulc-negative-k}\label{rule:ulc-first}
If $\cutsize < |X_0|$, terminate the current branch.
\end{redrule}
\begin{redrule}\label{rule:ulc-empty-phi}
If there exists a vertex $v \notin X_0$ with $\phi_v = \emptyset$ or $v \in S^\Psi$ and
$\Psi^S(v) \notin \phi_v$, then:
if $v \in S$, terminate the current branch, and otherwise
include $v$ into $X_0$.
\end{redrule}
\begin{redrule}\label{rule:separated-S}
If $G$ contains a connected component with vertex set $A$ and $A \subseteq S \setminus S^\Psi$,
invoke Lemma \ref{lem:ulc-propagate-labeling} to find a labeling of $G[A]$. If it exists,
add $A$ to $S^\Psi$ and extend $\Psi^S$ with the labeling found;
otherwise, terminate the current branch.
\end{redrule}
We note that Rule \ref{rule:ulc-negative-k} takes constant time to apply, Rule
\ref{rule:ulc-empty-phi} takes $O(n)$ time per vertex, and
each application of Rule \ref{rule:ulc-separated-S} takes $O(n^2)$ time
to search for all valid sets $A$ and $O(s^2|A|^2)$ time to apply the rule for one set $A$.

\begin{lemma}\label{lem:ulc-no-holes}
For any $v \in D \setminus X_0$
and any solution $(X,\Psi)$ to the tuple $(X_0,Y,Y^\Psi,\Psi^Y)$ of minimum 
possible $|X|$, if $v \in X$ then $N_G(v) \cap S \neq \emptyset$.
\end{lemma}
\begin{proof}
Asssume $v \in X$. We first claim that $N_G[v] \not\subseteq X$.
Indeed, otherwise, due to Steps \ref{step:ulc-initiate-branching} and \ref{step:ulc-cleaning},
  as $v \in D$ and $v \notin X_0$, we have $v \notin \bterms$
  and $\phi_v \neq \emptyset$, and
 $(X $let $\alpha \in \phi_v$ be an arbitrary element
  Assume otherwise
Assume otherwise $v \in X$ but $N_G(v) \cap S = \emptyset$.
\end{proof}

Moreover, for any $w \in C \cap X_\cP$, we cannot have $N_G(w) \subseteq X_\cP$.
Indeed, 
otherwise $(X_\cP \setminus \{w\}, \Psi_\cP \cup \{(w,\alpha)\})$
(for $\alpha = \cP(w)$ if $w \in \bterms$ or any $\alpha \in \phi_w$ otherwise),
is a solution to $\instance_b$ consistent with $\cP$ (as Rule \ref{rule:ulc-empty-phi}
    is not applicable) and $X_\cP \setminus \{w\}$
is interrogated by $S$ as $q > 1$ and $w$ is an isolated vertex in
$G \setminus (X_\cP \setminus \{w\})$, and we have a contradiction with the minimality
of $|X_\cP|$.
Therefore $C$ consists of some small stains of $S^\smallcc$ and their neighbourhood
in $D^\smallcc$.


==> steiner-cut.tex <==
\section{FPT algorithm for \steinercut}\label{sec:steiner-cut}

In this section we sketch the fixed-parameter algorithm for \steinercut. The algorithm will be similar to the one sketched in
the illustration, so we concentrate on differences. Full description of the algorithm can be found in
Appendix~\ref{sec:full-steiner}. Again, we can assume that the graph given in the input is connected.

\subsection{Recursive understanding}

This phase is even simpler than the corresponding one in the illustration. In the border problem the graph is equipped with a
set $\bterms$ of at most $2k$ border terminals. The behavior on border terminals is expressed by a triple
$\cP=(\rel_b,Y_b,\numbcc_b)$. $\rel_b$ is an equivalence relation on $\bterms$ expressing, which border terminals are required
to be in the same connected components after removing the solution. $Y_b$ is a subset of $\bterms$ such that if $(u,v)\in
\rel_b$, then $u\in Y_b$ if and only if $v\in Y_b$. $Y_b$ expresses which border terminals are required to be in a connected
component that contains a terminal. Finally, $\numbcc_b$ denotes how many connected components after removing the solution
need to contain a terminal. If $\instance_b$ is an instance of the border problem, we say that $X\subseteq E(G)$ is a solution
to $(\instance_b,\cP)$ if $|X|\leq k$ and in $G\setminus X$ all these constraints expressed by $\cP$ are satisfied. The border
problem is defined in the same manner as in the illustration: for each behavior on the border terminals we have to output a
solution with minimum $|X|$, or $\bot$ if no solution exists. Note that we do not need to remember also the connectivity
outside, i.e., $E_b$. Intuitively, we can avoid it because the support of $\rel_b$ is bounded by $2k$, so after trimming the
instance to one side of the separation we do not risk uncontrolled partitioning of equivalence classes of $\rel_b$.

The recurrential application and simplification steps are very similar, so we omit the details in this sketch. If the
recursive understanding cannot be applied further, we know that the graph does not admit a $(q,k)$-good edge separation for
$q=2^{O(k\log k)}$.

\subsection{High connectivity phase}

The first part of the high connectivity phase can be done in exactly the same manner as in the illustration. We guess a member
$S$ of an appropriately chosen family $\randfamily$ given by Lemma~\ref{lem:random}, assuming that $S$ is disjoint with the
solution but contains spanning trees of all small connected components after removing the solution as well as, for every
vertex of the big component incident to an edge of the solution, a tree of size $q+1$ attached to it and contained in $C_0$.
 Having guessed $S$ correctly, it is safe to contract the edges of $S$ and identify all the vertices onto which more than $q$
vertices were contracted. Thus, we obtain the same structure as in the illustration: a core vertex $b$ and a number of
components $B_i$ attached to it, whose edge sets have to be either disjoint with the solution or entirely contained in it.

As previously, if $b$ is not a border terminal, then we guess the equivalence class (or its lack) of $\rel_b$, whose vertices
will be in the same connected component as $b$. Having fixed the alignment of $b$, we can immediately resolve all the
components $B_i$ that contain border terminals. Those that contain border terminals guessed not to be in the same component
with $b$ have to be included in the solution, whereas those containing terminals required to be reachable from $b$ need to be
disjoint with the solution. We are left with a number of components $B_i$, and using the least possible number of additional
edges we need to cut out a given number of components containing terminals. Each component $B_i$ can be described by two
numbers: $a_i$, the number of edges of $B_i$, and $b_i$, the number of terminals in $V(B_i)\setminus \{b\}$. Hence, we need to
minimize the sum of $a_i$ in a subset of components subject to obtaining a given sum of $b_i$. This can be done in polynomial
time via standard dynamic programming. We remark that we have to be careful about one technical detail: the equivalence class
guessed to be in the same connected component as $b$ might require a terminal, so it may happen that we need to make sure that
at least one component $B_i$ that contains a terminal is disjoint with the solution. Fortunately, this can be solved by adding
an additional binary dimension to the dynamic program, which keeps track whether some component $B_i$ containing a terminal
has been already chosen to be disjoint with the solution. Details can be found in Appendix~\ref{sec:full-steiner}.


==> ulc.tex <==
\section{FPT algorithm for \ulc}\label{sec:ulc}

In this section we present a brief sketch of the algorithm for \ulc. The full version with all the formal proofs can be found
in Appendix~\ref{sec:full-ulc}. In the following description we point out the difficulties that arise due to considering a
node-deletion variant, as well as means that we use to overcome them. In fact, the edge-deletion variant can be reduced to the
node-deletion variant via a simple polynomial parameterized transformation; see Appendix~\ref{sec:full-ulc} for an appropriate
reduction.

\defparproblemu{\ulc}{An undirected graph $G$, a finite alphabet $\Sigma$ of size $s$,
 an integer $\cutsize$, and for each edge $e \in E(G)$ and each its endpoint $v$ a permutation $\psi_{e,v}$ of $\Sigma$, such that
if $e = uv$ then $\psi_{e,u} = \psi_{e,v}^{-1}$.}{$\cutsize+s$}{Does there exist
a set $X \subseteq V(G)$ of size at most $\cutsize$ and a function
$\Psi: V(G) \setminus X \to \Sigma$ such that
for any $uv \in E(G \setminus X)$ we have $(\Psi(u),\Psi(v)) \in \psi_{uv,u}$?}

Relations $\psi_{e,u}$ are called {\em{edge constraints}}, function
$\Psi$ is called a {\em{labeling}} and set $X$ is the {\em{deletion set}}.
We can naturally extend the notion of labelings to subsets:
a labeling of a subset $S\subseteq V(G)$ is a function from $S$ to the alphabet
that respects all the constraints in $G[S]$.
Given a set $S$ one can check in $O(s^2n^2)$ time whether $S$ admits
a consistent labeling via a simple breadth-first search on each connected component.

In case of the edge-deletion problems we could simply contract edges determined to be useless. Since \ulc is a vertex-deletion
type of problem, when we decide that a vertex is not going to be a part of a solution, then we {\em{bypass}} this vertex. When
bypassing a vertex $v$, we remove it from the graph and for each pair of neighbors $u_1,u_2 \in N_G(v)$ the constraint
$\psi_{u_1u_2}$ needs to be restricted to simultaneously satisfy also $\psi_{vu_2,v} \circ \psi_{vu_1,u_1}$. For this reason,
in Appendix~\ref{sec:full-ulc} we consider a slightly more general version of the \ulc problem, where edge constraints are
partial permutations and each vertex has a list of available labels $\phi_v \subseteq \Sigma$. The additional
{\em{vertex constraints}}, as we call lists $\phi_v$, are due to the fact that a solution might remove all but one vertex of
$N(v)$, and then even the restricted edge constraints between vertices of $N(v)$ are not enough. Details can be found in
Appendix~\ref{sec:full-ulc}.

\subsection{Good cuts in the node-deletion variant}

We need to adjust the notion of good separations also to the node-deletion problems. We gather formal definitions and proofs
on good separations in node-deletion setting in Appendix~\ref{sec:node-cuts}; the definitions there are slightly more general,
as they are adjusted to work also for the technical details of the algorithm for the \nmwcushort problem. Unfortunately, due
to technical difficulties we need two different notions of separations. The first one is a natural extension of the
corresponding definition in the edge-deletion variant.

\begin{definition}
Let $G$ be a connected graph. A triple $(Z,V_1,V_2)$ of subsets of $V(G)$ is called
a $(q,\cutsize)$-{\em{good node separation}}, if $|Z| \leq \cutsize$, $V_1$ and $V_2$ are vertex sets
of two different connected components of $G \setminus Z$ and $|V_1|,|V_2| > q$.
\end{definition}

Similarly to edge-deletion variant, one can find in time $O(2^{O(\min(q,\cutsize) \log (q + \cutsize))} n^3 \log n)$ a
$(q,\cutsize)$-good node separation in the graph, or conclude that no such exists. The second notion, called $(q,k)$-flower
separation, tries to capture the situation, where a large number of small components is attached to a common, small interface
(for a formal definition, see Appendix~\ref{sec:node-cuts}). Again, there exists an $O(2^{O(\min(q,\cutsize) \log (q +
\cutsize))} n^3 \log n)$ algorithm that either finds a $(q,\cutsize)$-flower separation, or concludes that no such exists. If
a graph does not admit a $(q,\cutsize)$-good node separation or a $(q,\cutsize)$-flower separation, we can prove a
similar result to Lemma~\ref{lem:high-structure} that encapsulates the high-connectivity behavior in $G$ (a more general result is proven as Lemma~\ref{lem:node-no-separation} in Appendix~\ref{sec:node-cuts}).

\begin{lemma}\label{lem:node-no-separation-body}
If a connected graph $G$ with terminals $\bterms \subseteq V(G)$
does not contain a $(q,\cutsize)$-good node separation or
a $(q,\cutsize)$-flower separation w.r.t. $\bterms$ then,
  for any $Z \subseteq V(G)$ of size at most $\cutsize$,
the graph $G \setminus Z$ contains at most $(2q+2)(2^\cutsize-1) + |\bterms| + 1$ connected components,
out of which at most one has more than $q$ vertices.
\end{lemma}

Note that the number of connected components could not be bounded if we only used the first type of separations. This problem
is the sole purpose of introducing flower separations as well. Fortunately, they admit enough structure to make the recursive
understanding step still work.

\subsection{Border problem and recursive understanding}

The definition of the border problem is very natural. In the border problem the graph is also equipped with a set $\bterms$ of
at most $4k$ border terminals. The behavior on the border terminals is expressed by a function $\cP:\bterms\to \Sigma \cup
\{\skull\}$, which simply fixes the values of the labeling. We say that a solution $(X,\Psi)$ is {\emph{consistent with}}
$\cP$ if $X \cap \bterms = \cP^{-1}(\skull)$ and $\Psi|_{\bterms \setminus X} = \cP|_{\bterms \setminus X}$.

\defproblemoutput{\bulc}{A \ulc{} instance
$\instance = (G,\Sigma,\cutsize,(\phi_v)_{v \in V(G)}, (\psi_{e,v})_{e \in E(G),v \in e})$
  with $G$ being connected,
and a set $\bterms \subseteq V(G)$ of size at most $4\cutsize$.}{
For each $\cP \in \mathbb{P}(\instance)$, output a solution $\sol_\cP = (X_\cP,\Psi_\cP)$
  to the instance $\instance$ that is consistent with $\cP$ and $|X_\cP|$
  is minimum possible, or outputs $\sol_\cP = \bot$ if such a pair does not exist.}

This definition allows a standard recursive understanding routine. Take $q = \cutsize(s+1)^{4\cutsize} + 2\cutsize$ and
suppose we are given a $(q,2k)$-good node separation $(Z,V_1,V_2)$ of $G$. At least one set $V_1,V_2$ has at most $2k$
terminals, let it be $V_1$. We recursively apply the algorithm to the instance trimmed to the graph induced by the set
$N[V_1]\subseteq V_1\cup Z$, where we also incorporate $N(V_1)\subseteq Z$ to the border terminals. Let us mark all the border
terminals and all the vertices that appeared in any output solution. One can easily show that all the unmarked vertices can be
safely bypassed, as their usage can be always replaced with using some marked ones. As we chose $q$ to be large enough, we
bypass at least one vertex and we obtain a recurrential equation that gives the claimed complexity bound. Given a
$(q,k)$-flower separation with respect to $\bterms$ we can make a recursive understanding step in the same manner. Once
neither a $(q,2k)$-good node separation nor a $(q,k)$-flower separation with respect to $\bterms$ is present, the graph admits
the structure expressed by Lemma~\ref{lem:node-no-separation-body} and we may proceed to the high connectivity phase. Note
that we also excluded good node separations with larger cutsets, as it will be useful in the future.

\subsection{High connectivity phase}

Recall that we are to compute the optimal solution for every behavior $\cP$ on border terminals. We iterate through all
possible $\cP$ and perform computation for each separately; note that this gives $2^{O(k\log s)}$ overhead to the running
time. From now on we can assume that $\cP$ is fixed.

Let us examine the structure of the instance after removing an optimal deletion set $X$, given by
Lemma~\ref{lem:node-no-separation-body}. We have at most $d=(q+1)(2^\cutsize-1) + 4\cutsize$ small components, each containing
at most $q$ vertices, and one component of unbounded size. Note that we can assume that this big component, denote its vertex
set by $\bigcc(X)$, contains more than $q$ vertices, as otherwise the whole graph has size at most $q(d+1)$ and a brute-force
search runs within the claimed complexity bound. As feasibility of an empty deletion set can be checked in polynomial time, we
assume that $X$ is nonempty. Let $\Psi$ be a labeling witnessing that $X$ is a feasible deletion set.

We now would like to use a similar approach to the one presented in the illustration, that is, to condensate the
high-connectivity behavior in $G$. Let us take $A_1$ to be the union of vertex sets of small connected components in
$G\setminus X$; note that $|A_1|\leq qd$. For every $u\in X\cap N(\bigcc(X))$ we construct a set $A^u\subseteq \bigcc(X)$ such
that $|A^u|=q+1$, $G[A^u]$ is connected and $A^u$ contains a neighbor of $u$; note that this is possible due to
$|\bigcc(X)|>q$. Let us now take $A_2=\bigcup_{u\in X\cap N(\bigcc(X))} A^u$; note that $|A_2|\leq k(q+1)$. Therefore, if
using Lemma~\ref{lem:random} we generate the random family $\randfamily$ for universe $U=V(G)$ and constants $a=qd+k(q+1)$,
$b=k$, then we know that there is a set $S_0\in \randfamily$ such that $A_1\cup A_2\subseteq S_0$ and $X\cap S_0=\emptyset$.
We guess the right $S_0$ by branching into $|\randfamily|$ subcases, labeled by $S\in \randfamily$. Formally, each branch
produces a candidate for an optimal solution and the algorithm picks the smallest possible; we argue that the branch with
$S_0$ guessed correctly produces an optimal solution. From now on, we have fixed a set $S$ and we seek a deletion set $X$ that
is disjoint with $S$, but $S$ contains all the vertex sets of small components after removing $X$, as well as, for every $u\in
X$ adjacent to the big component, a vertex set inducing a connected subgraph of size at least $q+1$ adjacent to $u$.

We refer to vertex sets of connected components of $G[S]$ as {\emph{stains}}; note that these sets will induce connected
subgraphs even after removing the solution. A stain is {\emph{big}} if it is of size at least $q+1$, otherwise it is
{\emph{small}}. Note that each big stain has to be entirely contained in $\bigcc(X)$. Moreover, for each stain there must
exist a consistent labeling of it, or otherwise we may immediately terminate the branch. We would like to mimic the
identification step from the illustration for big stains. Consider two big stains $C_1,C_2$. As the graph does not admit a
$(q,2k)$-good node separation, by Menger's theorem we can distinguish $2k+1$ paths $P^0,P^1,\ldots,P^{2k}$ from $C_1$ to $C_2$
that are internally vertex-disjoint. Having fixed $\Psi|_{C_1}$ (recall that we assume that all the vertices of $S$ do not
belong to $X$), for every path $P^i$ we can find a labeling $\Psi^i$ of $C_2$ that is $\Psi$ propagated via the path $P^i$ to
$C_2$ assuming that $P^i$ is not hit by the deletion set, or conclude that $P^i$ must be hit. As at most $k$ paths $P^i$ are
hit, majority of the paths are not hit. It follows that for these paths $\Psi^i=\Psi|_{C_2}$. Therefore, having fixed a
labeling on one big stain, we can also fix the labeling on all the big stains, even if we do not know the deletion set: for
each big stain we just compute all the labelings $\Psi^i$ and take the one that appears most of the time. Let $S^\bigcc$ be
the union of all big stains. We branch into at most $s$ branches, in each fixing a labeling of one vertex from $S^\bigcc$,
thus fixing the labeling of the whole $S^\bigcc$.

Denote $D^\bigcc=N(S^\bigcc)$; note that $D^\bigcc\cap S=\emptyset$. By our assumptions on $S$, we know that $X\cap
N(\bigcc(X))\subseteq D^\bigcc$. Intuitively, $S^\bigcc$ together with $D^\bigcc$ play the role of the core vertex $b$, while
the components of $G\setminus (S^\bigcc\cup D^\bigcc)$ can be solved more or less independently. In fact, it still holds that
for each such component, let $C$ be its vertex set, either $C$ is disjoint with $X$ and entirely contained in $\bigcc(X)$, or
all the small stains in $C$ are separated from each other and from $\bigcc(X)$ by $X$, while the deletion set $X$ contains
$C\setminus S$ as well as the whole $N(C)$. This corresponds to the observation in the edge-deletion variant, that no
component of the graph after removing the core has a nontrivial intersection with the deletion set.

We now construct an optimal deletion set by iteratively considering components of $G\setminus (S^\bigcc\cup D^\bigcc)$ and for
each trying to consistently label it. Recall that we begin with $S^\bigcc$ already labeled. Let $C$ be the vertex set of the
next component. If the whole $N(C)$ is already included in the deletion set, small stains contained in $C$ are already
separated from $\bigcc(X)$ so we can simply include the whole $C\setminus S$ to the deletion set and label all the remaining
small stains arbitrarily. Otherwise, let $C^\ast=G[S^\bigcc \cup N[C]]$ be the graph induced by $C$, $S^\bigcc$ and the subset
of $D^\bigcc$ that is adjacent to both of them. There are three possibilities:
\begin{itemize}
\item The labeling produced so far can be consistently extended on the whole $V(C^\ast)$, excluding vertices already
    chosen to the deletion set. In this case it is not hard to prove that it is safe to simply label $C$ with this
    labeling and proceed to the next component.
\item Even $G[C]$ cannot be consistently labeled. We infer that $C$ is disjoint with $\bigcc(X)$ and $C\setminus S$ as
    well as $N(C)$ has to be entirely in the deletion set, so we include $C\setminus S$ and $N(C)$ to the constructed
    deletion set, label the remaining small stains in $G[C\cap S]$ arbitrarily and proceed. Note that in this manner we
    strictly increase the size of the constructed deletion set, as $N(C)$ was not entirely contained in the so far
    constructed deletion set.
\item There exist some consistent labelings of $G[C]$, but none of them can be extended to vertices of $N(C)\subseteq
    D^\bigcc$ that are not yet included into the deletion set, so that it is consistent with already labeled vertices. We
    branch into several subcases:
\begin{itemize}
\item Either $C$ is disjoint with $\bigcc(X)$; in this branch we proceed as in the previous point.
\item Otherwise, we create a branch for every labeling of $G[C]$ (note that there are at most $s$ of them). In the
    corresponding branch we label $C$ accordingly. Moreover, as the labeling cannot be consistently extended to
    vertices of $N(C)$ that are not yet included in the deletion set, it follows that one can find just at most two
    vertices that are creating the problem. More precisely, in polynomial time one can find a set $B\subseteq N(C)$ of
    at most two vertices that are not yet included in the deletion set, such that the current labeling cannot be
    extended even to $B$. At least one vertex of $B$ has to be included in the deletion set, so we branch further into
    at most two subcases, in each including one of them.
\end{itemize}
\end{itemize}
Once we have dealt with all the components of $G\setminus (S^\bigcc\cup D^\bigcc)$, the set of vertices unlabeled so far is a
subset of $D^\bigcc$, which is dominated by $S^\bigcc$. Again, we can use the same observation that if the labeling cannot be
extended consistently on the whole remaining graph, there are just two vertices causing a problem, and the algorithm can
branch which of them to delete.

Note that in the whole procedure we produce at most $2s+1$ branches, and in each the size of the constructed deletion set
increases. Thus, the branching routine works in $O((2s+1)^k(ns)^{O(1)})$ time. For detailed analysis, see
Appendix~\ref{sec:full-ulc}.

